ScatterNeRF: Seeing Through Fog with Physically-Based Inverse Neural Rendering

Vision in adverse weather conditions, whether it be snow, rain, or fog is challenging. In these scenarios, scattering and attenuation severly degrades image quality. Handling such inclement weather conditions, however, is essential to operate autonomous vehicles, drones and robotic applications where human performance is impeded the most. A large body of work explores removing weather-induced image degradations with dehazing methods. Most methods rely on single images as input and struggle to generalize from synthetic fully-supervised training approaches or to generate high fidelity results from unpaired real-world datasets. With data as bottleneck and most of today's training data relying on good weather conditions with inclement weather as outlier, we rely on an inverse rendering approach to reconstruct the scene content. We introduce ScatterNeRF, a neural rendering method which adequately renders foggy scenes and decomposes the fog-free background from the participating media-exploiting the multiple views from a short automotive sequence without the need for a large training data corpus. Instead, the rendering approach is optimized on the multi-view scene itself, which can be typically captured by an autonomous vehicle, robot or drone during operation. Specifically, we propose a disentangled representation for the scattering volume and the scene objects, and learn the scene reconstruction with physics-inspired losses. We validate our method by capturing multi-view In-the-Wild data and controlled captures in a large-scale fog chamber.

==> sections/method_old.tex <==
\section{Neural Forward Model}

The color for each pixel is obtained by estimating the integral along the ray that starts from the camera origin and goes through the pixel:
\begin{equation}
\hat{C}_c(\mathbf{r}) = \int_{t_n}^{t_f} T_c(t) \sigma_c(\mathbf{r}(t)) \mathbf{c}_c(\mathbf{r}(t),\mathbf{d}) dt \ ,
\end{equation}
with
 \begin{equation}
 T_c(t) = exp \left( -\int_{t_n}^{t} \sigma_c(\mathbf{r}(s)) ds \right)
 \end{equation}
In practice, the integral is estimated using quadrature, leading to:
\begin{equation}
\label{eqn:nerf_approx_1}
\hat{C}_c(\mathbf{r}) = \sum_{i}^{N} w_{c_i} \mathbf{c}_{c_i} ,
\end{equation}

where $\delta_i = t_{t+1} - t_i$ and :
\begin{equation}
\label{eqn:nerf_approx_2}
w_{c_i} = T_{c_i} (1-exp(\sigma_{c_i} \delta_i ))
\end{equation}
\begin{equation}
\label{eqn:nerf_approx_3}
T_{c_i}= exp \left( -\sum_{j=1}^{i-1} \sigma_{c_j} \delta_j \right)
\end{equation}

To learn a better representation, two networks $f_{c_{coarse}}$ and $f_{c_{fine}}$ are learned simultaneously, with the same objective function but different sampling procedure. \newline
For the participating media, the MLP $f_p$ has the analogous function of estimating its color and density:
\begin{equation}
{\mathbf{c}_p,\sigma_p} = f_p \left( \gamma(\mathbf{x}), \gamma(\mathbf{d}) \right) 
\end{equation}
By sampling from both $f_c$ and $f_p$, the original scene $\textit{F}$ can be estimated. In fact, as one specific point $\mathbf{x}$ can not belong at the same time to the participating media and to the scene, the two events $\mathbf{x} \in \textit{C}$, $\mathbf{x} \in \textit{P}$ (i.e. belonging to the scene and belonging to the media) are disjoint and we can write :
\begin{equation}
\label{eqn:fog_volumetric_rendering2}
\begin{split}
\hat{C}_F(\mathbf{r}) =\int_{t_n}^{t_f} T_F(t) & ( \sigma_p(\mathbf{r}(t)) \mathbf{c}_p(\mathbf{r}(t),\mathbf{d}) \\
&+ \sigma_c(\mathbf{r}(t)) \mathbf{c}_c(\mathbf{r}(t),\mathbf{d}) )  dt \     
\end{split}
\end{equation}
where:
 \begin{equation}
\label{eqn:fog_T}
 T_F(t) = exp \left( -\int_{t_i}^{t} \sigma_p(\mathbf{r}(s)) +\sigma_c(\mathbf{r}(s)) ds \right)
 \end{equation}

 Similarly to the original formula, we can use quadrature (full derivation in the supplement materials) to estimate the integral as:
 \begin{equation}
 \label{eqn:fog_C_discrete}
\hat{C}_F(\mathbf{r}) = \sum_{i}^{N} T_{F_i} (1-exp( (\sigma_{c_i} +\sigma_{p_i} )\delta_i )) \left( \frac{\sigma_{c_i}}{\sigma_{F_i}} \mathbf{c}_{c_i} + \frac{\sigma_{p_i}}{\sigma_{F_i}} \mathbf{c}_{p_i} \right) ,
\end{equation}
where :
\todo{This is not identical to my notes. Can you send me the new derivation to crosscheck?} \reply{See at the bottom}
\begin{equation}
\label{eqn:fog_T_discrete}
T_{F_i}= exp \left( -\sum_{j=1}^{i-1} (\sigma_{c_j}+\sigma_{p_j}) \delta_j \right)
\end{equation}
This result can be interpreted as the standard formulation used for NeRF (i.e. \ref{eqn:nerf_approx_1}, \ref{eqn:nerf_approx_2}, \ref{eqn:nerf_approx_3} ) by having $\sigma_{F_i} = \sigma_{p_i} + \sigma_{c_i}$ and $\mathbf{c}_{F_i} = \left( \frac{\sigma_{c_i}}{\sigma_{F_i}} \mathbf{c}_{c_i} + \frac{\sigma_{p_i}}{\sigma_{F_i}} \mathbf{c}_{p_i} \right) $ :
 \begin{equation}
\hat{C}_F(\mathbf{r}) = \sum_{i}^{N} T_{F_i} (1-exp(\sigma_{F_i} \delta_i )) \mathbf{c}_{F_i} ,
\end{equation}
\begin{equation}
T_{F_i}= exp \left( -\sum_{j=1}^{i-1} \sigma_{F_j} \delta_j \right)
\end{equation}

Instead of employing a coarse and fine MLP for the particiapting media as well, we only use a single MLP $f_p$ given the limited spatial variance of media color and density. \newline
Please note that, compared to the original model, the only required additional step is to query a different MLP for the already-sampled points, making this framework lightweight both in memory and computation terms. \newline


==> tables/results_dehazing.tex <==
\begin{table}[!tp]
    \footnotesize
    \setlength{\tabcolsep}{2pt} % general space between cols (6pt standard)
    \setlength\extrarowheight{2pt}
    \centering
    \resizebox{.49\textwidth}{!}{
    \begin{tabular}{@{}lccccccccc@{}}
            \toprule
            & \multicolumn{6}{|c|}{\textbf{\textsc{Rendering Methods}}} & \multicolumn{3}{|c|}{\textbf{\textsc{Dehazing Methods}}} \\
             & ScatterNeRF & NeRF & NeRF++ & MipNeRF & MipNeRF360 & RefNeRF & ... & ZeroScatter & ...  \\ 
            \midrule
            LPIPS & \\
            PSNR & \\
            SSIM & \\
			% \multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{last}}}}}
			% \input{ScatterNerf/tables/results_last}\\
 		% 	\midrule
 		% 	\multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{random}}}}}
			% \input{ScatterNerf/tables/results_random}\\
			% \midrule
   %          \multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{left/right}}}}}
			% \input{ScatterNerf/tables/results_left_right}\\
			% \midrule
            \bottomrule
    \end{tabular}
    }
    \vspace*{-5pt}
    \caption{\small Quantitative performance comparison on controlled fog chamber measurements.
	\vspace*{-4mm}
}
    \label{tab:results_dehazing}
\end{table}

==> tables/results_foggy_reconstruction.tex <==
\begin{table*}[!tp]
    \footnotesize
    \setlength{\tabcolsep}{6pt} % general space between cols (6pt standard)
    \setlength\extrarowheight{2pt}
    \centering
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{@{}lcccccccccccc@{}}
            \toprule
            & \multicolumn{6}{|c|}{\textbf{\textsc{Automotive Dataset}}} & \multicolumn{6}{|c|}{\textbf{\textsc{Fog Chamber Dataset}}} \\

            & \multicolumn{3}{|c|}{\textbf{random split}} & \multicolumn{3}{|c|}{\textbf{left/right split}} & \multicolumn{3}{|c|}{\textbf{random split foggy}} & \multicolumn{3}{|c|}{\textbf{random split clear}}\\
            \textbf{\textsc{Method}} & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM \\ 
            \midrule
			\input{tables/results_mean}\\
 		% 	\midrule
 		% 	\multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{random}}}}}
			% \input{ScatterNerf/tables/results_random}\\
			% \midrule
   %          \multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{left/right}}}}}
			% \input{ScatterNerf/tables/results_left_right}\\
			% \midrule
            \bottomrule
    \end{tabular}
    }
    \vspace*{-5pt}
    \caption{\small Quantitative comparison on foggy scene reconstruction of ScatterNerf and state-of-the-art rendering methods. We report LPIPS, PSNR, and SSIM for the proposed Automotive Dataset and the controlled Fog Chamber Dataset. Best results in each category are in \textbf{bold} and second best are \underline{underlined}. ScatterNeRF outperforms all other methods by learning to distinguish between scattered media and object colours. 
	\vspace*{-4mm}
}
\label{tab:results_foggy_reconstruction}
\end{table*}

==> tables/results_last.tex <==
& NeRF & \textbf{0.518} & \underline{26.9} & \textbf{0.852} & \textbf{0.521} & \textbf{28.61} & \textbf{0.92} & \underline{0.504} & \underline{26.98} & \underline{0.915} & \textbf{0.49} & 27.18 & 0.913 & \underline{0.495} & \underline{29.23} & 0.917 \\ 
& NeRF++ & \textbf{0.518} & 26.85 & 0.838 & 0.564 & 23.79 & 0.891 & \textbf{0.501} & \textbf{30.61} & \textbf{0.946} & 0.491 & \textbf{27.87} & \underline{0.924} & \textbf{0.489} & \textbf{30.78} & \textbf{0.926} \\ 
& Mip-NeRF & 0.592 & 23.25 & 0.817 & 0.574 & 23.29 & 0.881 & 0.568 & 22.79 & 0.894 & 0.534 & 26.66 & \textbf{0.927} & 0.537 & 26.3 & 0.899 \\ 
& Mip-NeRF360 & 0.563 & \textbf{26.94} & 0.823 & 0.546 & 24.03 & 0.896 & 0.538 & 26.94 & 0.896 & 0.522 & \underline{27.76} & 0.911 & 0.518 & 28.41 & 0.91 \\ 
& Plenoxels & 0.547 & 19.26 & \underline{0.843} & \underline{0.533} & 18.0 & 0.864 & 0.512 & 18.18 & 0.885 & \textbf{0.49} & 17.66 & 0.881 & 0.513 & 17.15 & 0.859 \\ 
& Ref-NeRF & 0.577 & 22.09 & 0.804 & 0.554 & \underline{26.47} & \underline{0.913} & 0.53 & 24.57 & 0.896 & 0.522 & 25.87 & 0.921 & 0.513 & 27.74 & \underline{0.921} 


==> tables/results_left_right.tex <==
& NeRF & \textbf{0.271} & 35.56 & \textbf{0.96} & \underline{0.341} & 37.17 & \textbf{0.968} & \textbf{0.285} & 36.74 & \textbf{0.975} & \textbf{0.279} & 36.68 & \textbf{0.973} & \textbf{0.289} & 36.73 & \textbf{0.972} \\ 
& NeRF++ & \underline{0.288} & \textbf{36.52} & \underline{0.956} & \underline{0.341} & \textbf{37.69} & \textbf{0.968} & \underline{0.301} & \textbf{37.45} & \underline{0.974} & \underline{0.291} & \textbf{37.28} & \underline{0.971} & \underline{0.303} & \textbf{37.5} & \underline{0.97} \\ 
& Mip-NeRF & 0.375 & 31.22 & 0.938 & 0.357 & 33.63 & 0.965 & 0.372 & 32.25 & 0.958 & 0.336 & 32.99 & 0.964 & 0.344 & 33.18 & 0.962 \\ 
& Mip-NeRF360 & 0.362 & 33.65 & 0.907 & \textbf{0.334} & 36.85 & 0.957 & 0.336 & 36.19 & 0.948 & 0.302 & 36.51 & 0.954 & 0.315 & \underline{36.75} & 0.954 \\ 
& Plenoxels & 0.475 & 31.58 & 0.916 & 0.486 & 31.58 & 0.942 & 0.472 & 30.22 & 0.94 & 0.488 & 29.49 & 0.93 & 0.486 & 30.41 & 0.937 \\ 
& Ref-NeRF & 0.385 & \underline{35.98} & 0.942 & 0.369 & \underline{37.67} & 0.967 & 0.383 & \underline{36.86} & 0.964 & 0.36 & \underline{37.13} & 0.967 & 0.402 & 36.67 & 0.961 \\ 
& Aug-NeRF & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
& ScatterNeRF & 0.21 & 37.66 & 0.97 & 0.283 & 38.16 & 0.974 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 

==> tables/results_left_right_v1.tex <==
& NeRF & \textbf{0.28} & \underline{36.81} & \textbf{0.974} & \textbf{0.241} & \underline{36.9} & \textbf{0.98} & \textbf{0.276} & \underline{36.93} & \textbf{0.976} & \underline{0.338} & \underline{35.82} & \textbf{0.958} & \textbf{0.296} & 37.37 & \textbf{0.977} \\ 
& NeRF++ & \underline{0.302} & \textbf{37.72} & \underline{0.972} & \underline{0.26} & \textbf{37.74} & \underline{0.979} & \underline{0.286} & \textbf{37.73} & \underline{0.975} & \textbf{0.337} & \textbf{36.72} & \textbf{0.958} & 0.316 & \textbf{38.15} & \underline{0.976} \\ 
& Mip-NeRF & 0.36 & 32.47 & 0.959 & 0.357 & 32.28 & 0.961 & 0.342 & 32.4 & 0.962 & 0.377 & 31.64 & 0.945 & 0.312 & 34.65 & 0.972 \\ 
& Mip-NeRF360 & 0.329 & 36.22 & 0.947 & 0.32 & 36.31 & 0.951 & 0.298 & 36.88 & 0.957 & 0.343 & 35.62 & 0.938 & \underline{0.305} & 37.45 & 0.966 \\ 
& Plenoxels & 0.475 & 30.8 & 0.94 & 0.451 & 29.77 & 0.936 & 0.458 & 31.2 & 0.942 & 0.485 & 30.14 & 0.925 & 0.473 & 30.86 & 0.944 \\ 
& Ref-NeRF & 0.38 & 36.71 & 0.962 & 0.373 & 36.88 & 0.965 & 0.359 & 36.86 & 0.967 & 0.41 & 35.05 & 0.95 & 0.338 & \underline{37.68} & 0.974 \\ 
& Aug-NeRF & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 

==> tables/results_mean.tex <==
NeRF & \underline{0.295} & \underline{41.67} & \underline{0.974} & \textbf{0.29} & 36.67 & \textbf{0.971} & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
NeRF++ & 0.305 & \textbf{41.97} & 0.972 & \underline{0.302} & \textbf{37.45} & \underline{0.97} & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
Mip-NeRF & 0.361 & 34.98 & 0.962 & 0.353 & 32.67 & 0.959 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
Mip-NeRF360 & 0.328 & 39.99 & 0.962 & 0.324 & 36.24 & 0.948 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
Plenoxels & 0.479 & 29.8 & 0.931 & 0.475 & 30.6 & 0.935 & \textbf{0.642} & \textbf{19.65} & \textbf{0.818} & \textbf{0.683} & \textbf{17.45} & \textbf{0.54} \\ 
Ref-NeRF & 0.368 & 40.2 & 0.964 & 0.376 & \underline{36.75} & 0.962 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\ 
Aug-NeRF & \textbf{0.218} & 39.98 & \textbf{0.979} & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 


==> tables/results_random.tex <==
& Aug-NeRF & 0.26 & 39.18 & 0.964 & 0.316 & 39.83 & 0.968 & 0.275 & 40.38 & 0.971 & 0.259 & 40.18 & 0.977 & 0.277 & 40.54 & 0.974 \\ 
& DVGO & 0.404 & 35.46 & 0.923 & 0.441 & 37.49 & 0.93 & 0.4 & 39.35 & 0.955 & 0.36 & 39.68 & 0.963 & 0.382 & 39.16 & 0.958 \\ 
& Mip-NeRF & 0.28 & 38.84 & 0.962 & 0.337 & 40.52 & 0.968 & 0.271 & 41.72 & 0.975 & 0.27 & 41.23 & 0.977 & 0.28 & 41.72 & 0.975 \\ 
& Mip-NeRF360 & \underline{0.222} & \underline{40.92} & \underline{0.971} & \textbf{0.28} & \underline{41.25} & \textbf{0.973} & \textbf{0.228} & \underline{42.17} & \underline{0.976} & \underline{0.244} & 41.91 & 0.977 & \textbf{0.247} & 42.2 & \underline{0.977} \\ 
& NeRF & 0.278 & 39.06 & 0.964 & 0.354 & 40.86 & 0.968 & 0.293 & 41.84 & 0.974 & 0.271 & 41.6 & \underline{0.978} & 0.293 & 42.39 & 0.976 \\ 
& NeRF++ & 0.288 & 39.54 & 0.962 & 0.36 & 41.07 & 0.966 & 0.306 & 42.11 & 0.972 & 0.293 & \underline{42.07} & 0.976 & 0.304 & \underline{42.41} & 0.974 \\ 
& Plenoxels & 0.476 & 30.9 & 0.91 & 0.498 & 32.28 & 0.939 & 0.478 & 29.93 & 0.934 & 0.486 & 28.29 & 0.928 & 0.489 & 29.34 & 0.934 \\ 
& Ref-NeRF & 0.4 & 36.64 & 0.94 & 0.377 & 39.85 & 0.966 & 0.377 & 40.53 & 0.964 & 0.343 & 40.47 & 0.972 & 0.366 & 41.13 & 0.967 \\ 
& ScatterNeRF & \textbf{0.22} & \textbf{41.45} & \textbf{0.975} & \underline{0.299} & \textbf{42.57} & \underline{0.972} & \underline{0.235} & \textbf{44.58} & \textbf{0.98} & \textbf{0.234} & \textbf{44.44} & \textbf{0.981} & \underline{0.253} & \textbf{43.88} & \textbf{0.978}


==> tables/results_random_v1.tex <==

& Aug-NeRF & 0.248 & 41.29 & \underline{0.979} & 0.242 & 41.75 & 0.981 & \underline{0.259} & 40.1 & 0.976 & 0.302 & 38.99 & 0.964 & 0.286 & 40.74 & 0.978 \\ 
& DVGO & 0.376 & 38.51 & 0.947 & 0.349 & 40.14 & 0.966 & 0.366 & 39.53 & 0.964 & 0.376 & 38.92 & 0.95 & 0.368 & 40.55 & 0.968 \\ 
& Mip-NeRF & 0.272 & 41.88 & 0.976 & 0.25 & 42.83 & 0.981 & 0.268 & 41.43 & \underline{0.977} & 0.321 & 40.2 & 0.963 & -1.0 & -1.0 & -1.0 \\ 
& Mip-NeRF360 & \underline{0.235} & 42.37 & 0.978 & \textbf{0.225} & 42.55 & 0.981 & \textbf{0.23} & \underline{42.01} & \textbf{0.979} & \underline{0.268} & \underline{41.53} & \underline{0.969} & \textbf{0.241} & 42.97 & \underline{0.981} \\ 
& NeRF & 0.287 & 41.84 & 0.975 & 0.256 & 43.67 & \underline{0.982} & 0.28 & 41.71 & \underline{0.977} & 0.332 & 40.36 & 0.962 & 0.305 & 43.39 & 0.979 \\ 
& NeRF++ & 0.292 & \underline{42.38} & 0.975 & 0.267 & \underline{43.82} & 0.98 & 0.29 & \textbf{42.04} & 0.976 & 0.336 & 40.69 & 0.962 & 0.312 & \underline{43.56} & 0.978 \\ 
& Plenoxels & 0.481 & 29.85 & 0.933 & 0.456 & 29.72 & 0.943 & 0.461 & 28.72 & 0.932 & 0.497 & 29.49 & 0.922 & 0.473 & 29.47 & 0.938 \\ 
& Ref-NeRF & 0.382 & 39.61 & 0.962 & 0.376 & 40.81 & 0.967 & 0.352 & 40.13 & 0.969 & 0.365 & 40.04 & 0.96 & 0.339 & 42.81 & 0.976 \\ 
& ScatterNeRF & \textbf{0.231} & \textbf{44.45} & \textbf{0.981} & \underline{0.228} & \textbf{45.27} & \textbf{0.983} & -1.0 & -1.0 & -1.0 & \textbf{0.255} & \textbf{42.96} & \textbf{0.973} & \underline{0.265} & \textbf{44.64} & \textbf{0.982}


==> tables/results_table_old.tex <==
\begin{table*}[!tp]
    \footnotesize
    \setlength{\tabcolsep}{4pt} % general space between cols (6pt standard)
    \setlength\extrarowheight{2pt}
    \centering
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{@{}clccccccccccccccc@{}}
            \toprule
            && \multicolumn{3}{|c|}{\textbf{Sequence00}} & \multicolumn{3}{|c|}{\textbf{Sequence04}} & \multicolumn{3}{|c|}{\textbf{Sequence06}} & \multicolumn{3}{|c|}{\textbf{Sequence08}} & \multicolumn{3}{|c|}{\textbf{Sequence09}}\\
            & \textbf{\textsc{Method}} & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM \\ 
            \midrule
			\multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{last}}}}}
			\input{tables/results_last}\\
 			\midrule
 			\multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{random}}}}}
			\input{tables/results_random}\\
			\midrule
            \multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{left/right}}}}}
			\input{tables/results_left_right}\\
			\midrule
            \bottomrule
    \end{tabular}
    }
    \vspace*{-5pt}
    \caption{\label{tab:results}\small Comparison of the proposed ScatterNerf and state-of-the-art methods on the different test datasets. Best results in each category are in \textbf{bold} and second best are
    \underline{underlined}.
	\vspace*{-4mm}
}
\end{table*}

==> tables/results_table_v1.tex <==
\begin{table*}[!tp]
    \footnotesize
    \setlength{\tabcolsep}{4pt} % general space between cols (6pt standard)
    \setlength\extrarowheight{2pt}
    \centering
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{@{}clccccccccccccccc@{}}
            \toprule
            && \multicolumn{3}{|c|}{\textbf{Sequence10}} & \multicolumn{3}{|c|}{\textbf{Sequence11}} & \multicolumn{3}{|c|}{\textbf{Sequence12}} & \multicolumn{3}{|c|}{\textbf{Sequence13}} & \multicolumn{3}{|c|}{\textbf{Sequence14}}\\
            & \textbf{\textsc{Method}} & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM \\
            \midrule
 			\multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{random}}}}}
			\input{tables/results_random_v1}\\
			\midrule
            \multirow{6}{*}{\rotatebox[origin=l]{90}{\parbox[c]{1.6cm}{\centering \textbf{\small{left/right}}}}}
			\input{tables/results_left_right_v1}\\
			\midrule
            \bottomrule
    \end{tabular}
    }
    \vspace*{-5pt}
    \caption{\label{tab:results}\small Comparison of the proposed ScatterNerf and state-of-the-art methods on the different test datasets. Best results in each category are in \textbf{bold} and second best are
    \underline{underlined}.
	\vspace*{-4mm}
}
\end{table*}
